Imagined Rollouts are Kinematic, Not Dynamic: A Diagnosis of Long-Horizon World-Model Failure

Long-horizon failure in world models is conventionally attributed to compounding error, a generic framing that does not distinguish what kind of error compounds. We propose a kinematic-vs-dynamic reframing: world models tend to imagine kinematically rather than dynamically. We operationalize this as the imagined Kinematic-Consistency Error, a per-step diagnostic that measures how far a rollout departs from a closed-form kinematic null, paired with a perturbation protocol that tests whether iKCE responds when physical conditions cross a regime boundary. We instantiate the diagnostic on a released DreamerV3 checkpoint trained on DMC walker-walk, where imagined iKCE runs roughly two orders of magnitude above that of matched real-physics rollouts. Across a friction sweep that crosses the gait-collapse boundary, the model's iKCE stays statistically flat even as the trained policy's reward collapses through the same range, providing the kinematic-not-dynamic signature. The diagnostic distinguishes kinematic from dynamic imagination at horizons longer than the embodiment's gait period.

==> tex/headline_gait_a64.tex <==
% Ablation figure — h=64-trained actor checkpoint, gait DOFs view.
\drawiKCEheadline
  {walker_walk_physics_policy_gait_a64}
  {walker_walk_wm_gait_a64}
  {{walker gait DOFs, $T{=}64$, actor $h{=}64$}}
  {0.20}
  {ymode=linear, ymin=0.8, ymax=2.1,
   legend style={at={(0.98, 0.98)}, anchor=north east}}


==> tex/headline_gait_h16.tex <==
% Headline figure, gait-DOF view, measurement horizon T=16.
\drawiKCEheadline
  {walker_walk_physics_policy_gait}
  {walker_walk_wm_gait}
  {{walker gait DOFs, $T{=}16$}}
  {0.20}
  {ymode=linear, ymin=0.8, ymax=2.1,
   legend style={at={(0.98, 0.98)}, anchor=north east}}


==> tex/headline_identity_h16.tex <==
% Headline figure, identity view (z, vz), measurement horizon T=16.
% Short-horizon control: friction signal does not surface here on either side.
\drawiKCEheadline
  {walker_walk_physics_policy}
  {walker_walk_wm}
  {{$(z, v_z)$, $T{=}16$}}
  {0.20}
  {ymode=log, ymin=2e-5, ymax=1e-2}

